FOCA: A Methodology for Ontology Evaluation

Modeling an ontology is a hard and time-consuming task. Although methodologies are useful for ontologists to create good ontologies, they do not help with the task of evaluating the quality of the ontology to be reused. For these reasons, it is imperative to evaluate the quality of the ontology after constructing it or before reusing it. Few studies usually present only a set of criteria and questions, but no guidelines to evaluate the ontology. The effort to evaluate an ontology is very high as there is a huge dependence on the evaluator's expertise to understand the criteria and questions in depth. Moreover, the evaluation is still very subjective. This study presents a novel methodology for ontology evaluation, taking into account three fundamental principles: i) it is based on the Goal, Question, Metric approach for empirical evaluation; ii) the goals of the methodologies are based on the roles of knowledge representations combined with specific evaluation criteria; iii) each ontology is evaluated according to the type of ontology. The methodology was empirically evaluated using different ontologists and ontologies of the same domain. The main contributions of this study are: i) defining a step-by-step approach to evaluate the quality of an ontology; ii) proposing an evaluation based on the roles of knowledge representations; iii) the explicit difference of the evaluation according to the type of the ontology iii) a questionnaire to evaluate the ontologies; iv) a statistical model that automatically calculates the quality of the ontologies.

==> referencias <==
% This file was created with JabRef 2.10.
% Encoding: Cp1252


@Article{berners2001semantic,
  Title                    = {The semantic web},
  Author                   = {Berners-Lee, Tim and Hendler, James and Lassila, Ora and others},
  Journal                  = {Scientific american},
  Year                     = {2001},
  Number                   = {5},
  Pages                    = {28--37},
  Volume                   = {284},

  Publisher                = {New York, NY, USA:}
}

@Article{davis1993knowledge,
  Title                    = {What is a knowledge representation?},
  Author                   = {Davis, Randall and Shrobe, Howard and Szolovits, Peter},
  Journal                  = {AI magazine},
  Year                     = {1993},
  Number                   = {1},
  Pages                    = {17},
  Volume                   = {14}
}

@Article{espinheira2015prediction,
  Title                    = {Prediction Measures in Beta Regression Models},
  Author                   = {Espinheira, Patr{\'\i}cia L and da Silva, Luana Cec{\'\i}lia Meireles and Silva, Alisson de Oliveira},
  Journal                  = {arXiv preprint arXiv:1501.04830},
  Year                     = {2015}
}

@Article{fernandez1997methontology,
  Title                    = {Methontology: from ontological art towards ontological engineering},
  Author                   = {Fern{\'a}ndez-L{\'o}pez, Mariano and G{\'o}mez-P{\'e}rez, Asunci{\'o}n and Juristo, Natalia},
  Year                     = {1997},

  Publisher                = {American Asociation for Artificial Intelligence}
}

@Article{ferrari2004beta,
  Title                    = {Beta regression for modelling rates and proportions},
  Author                   = {Ferrari, Silvia and Cribari-Neto, Francisco},
  Journal                  = {Journal of Applied Statistics},
  Year                     = {2004},
  Number                   = {7},
  Pages                    = {799--815},
  Volume                   = {31},

  Publisher                = {Taylor \& Francis}
}

@Article{gomez2001evaluation,
  Title                    = {Evaluation of ontologies},
  Author                   = {G{\'o}mez-P{\'e}rez, Asunci{\'o}n},
  Journal                  = {International Journal of intelligent systems},
  Year                     = {2001},
  Number                   = {3},
  Pages                    = {391--409},
  Volume                   = {16},

  Publisher                = {Wiley Online Library}
}

@Book{gangemi2006modelling,
  Title                    = {Modelling ontology evaluation and validation},
  Author                   = {Gangemi, Aldo and Catenacci, Carola and Ciaramita, Massimiliano and Lehmann, Jos},
  Publisher                = {Springer},
  Year                     = {2006}
}

@Article{gruninger1995methodology,
  Title                    = {Methodology for the Design and Evaluation of Ontologies},
  Author                   = {Gr{\"u}ninger, Michael and Fox, Mark S},
  Year                     = {1995},

  Publisher                = {Citeseer}
}

@Article{gruber1995toward,
  Title                    = {Toward principles for the design of ontologies used for knowledge sharing?},
  Author                   = {Gruber, Thomas R},
  Journal                  = {International journal of human-computer studies},
  Year                     = {1995},
  Number                   = {5},
  Pages                    = {907--928},
  Volume                   = {43},

  Publisher                = {Elsevier}
}

@Article{gruber1993translation,
  Title                    = {A translation approach to portable ontology specifications},
  Author                   = {Gruber, Thomas R},
  Journal                  = {Knowledge acquisition},
  Year                     = {1993},
  Number                   = {2},
  Pages                    = {199--220},
  Volume                   = {5},

  Publisher                = {Elsevier}
}

@Book{guarino1998formal,
  Title                    = {Formal ontology in information systems: Proceedings of the first international conference (FOIS'98), June 6-8, Trento, Italy},
  Author                   = {Guarino, Nicola},
  Publisher                = {IOS press},
  Year                     = {1998},
  Volume                   = {46}
}

@Article{kotis2006human,
  Title                    = {Human-centered ontology engineering: The HCOME methodology},
  Author                   = {Kotis, Konstantinos and Vouros, George A},
  Journal                  = {Knowledge and Information Systems},
  Year                     = {2006},
  Number                   = {1},
  Pages                    = {109--131},
  Volume                   = {10},

  Publisher                = {Springer}
}

@Article{mena2009scriptlattes,
  Title                    = {ScriptLattes: an open-source knowledge extraction system from the Lattes platform},
  Author                   = {Mena-Chalco, Jes{\'u}s Pascual and Junior, Cesar and Marcondes, Roberto},
  Journal                  = {Journal of the Brazilian Computer Society},
  Year                     = {2009},
  Number                   = {4},
  Pages                    = {31--39},
  Volume                   = {15},

  Publisher                = {SciELO Brasil}
}

@InCollection{obrst2007evaluation,
  Title                    = {The evaluation of ontologies},
  Author                   = {Obrst, Leo and Ceusters, Werner and Mani, Inderjeet and Ray, Steve and Smith, Barry},
  Booktitle                = {Semantic Web},
  Publisher                = {Springer},
  Year                     = {2007},
  Pages                    = {139--158}
}

@InProceedings{thomasson2004methods,
  Title                    = {Methods of categorization},
  Author                   = {Thomasson, Amie L},
  Booktitle                = {Proceedings of the 3rd International Conference (FOIS'04)},
  Year                     = {2004},
  Pages                    = {3--16}
}

@Book{vrandevcic2009ontology,
  Title                    = {Ontology evaluation},
  Author                   = {Vrande{\v{c}}i{\'c}, Denny},
  Publisher                = {Springer},
  Year                     = {2009}
}


